Output Feedback Controller Design with Symbolic Observers for Cyber-physical Systems

In this paper, we design a symbolic output feedback controller of a cyber-physical system (CPS). The physical plant is modeled by an infinite transition system. We consider the situation that a finite abstracted system of the physical plant, called a c-abstracted system, is given. There exists an approximate alternating simulation relation from the c-abstracted system to the physical plant. A desired behavior of the c-abstracted system is also given, and we have a symbolic state feedback controller of the physical plant. We consider the case where some states of the plant are not measured. Then, to estimate the states with abstracted outputs measured by sensors, we introduce a finite abstracted system of the physical plant, called an o-abstracted system, such that there exists an approximate simulation relation. The relation guarantees that an observer designed based on the state of the o-abstracted system estimates the current state of the plant. We construct a symbolic output feedback controller by composing these systems. By a relation-based approach, we proved that the controlled system approximately exhibits the desired behavior.

==> eptcsdata.tex <==
\providecommand{\firstpage}{37}
\providecommand{\publicationstatus}{Kargahi and Trivedi: Verification and Validation of \\Cyber-Physical Systems 2016 (V2CPS-16)\\
EPTCS 232, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.232.7}{10.4204/EPTCS.232.7}}
\pdfoutput=1

